A new measure between sets of probability distributions with applications to erratic financial behavior

This paper introduces a new framework to quantify distance between finite sets with uncertainty present, where probability distributions determine the locations of individual elements. Combining this with a Bayesian change point detection algorithm, we produce a new measure of similarity between time series with respect to their structural breaks. First, we demonstrate the algorithm's effectiveness on a collection of piecewise autoregressive processes. Next, we apply this to financial data to study the erratic behavior profiles of 19 countries and 11 sectors over the past 20 years. Our measure provides quantitative evidence that there is greater collective similarity among sectors' erratic behavior profiles than those of countries, which we observe upon individual inspection of these time series. Our measure could be used as a new framework or complementary tool for investors seeking to make asset allocation decisions for financial portfolios.

==> Journal_macros.tex <==
Short form of journal title&Macro name&Short form of journal title&Macro name\\
\mr
2D Mater.&\verb"\TDM"&Mater. Res. Express&\verb"\MRE"\\
Biofabrication&\verb"\BF"&Meas. Sci. Technol.$^c$&\verb"\MST"\\
Bioinspir. Biomim.&\verb"\BB"&Methods Appl. Fluoresc.&\verb"\MAF"\\
Biomed. Mater.&\verb"\BMM"&Modelling Simul. Mater. Sci. Eng.&\verb"\MSMSE"\\
Class. Quantum Grav.&\verb"\CQG"&Nucl. Fusion&\verb"\NF"\\
Comput. Sci. Disc.&\verb"\CSD"&New J. Phys.&\verb"\NJP"\\
Environ. Res. Lett.&\verb"\ERL"&Nonlinearity$^{a,b}$&\verb"\NL"\\
Eur. J. Phys.&\verb"\EJP"&Nanotechnology&\verb"\NT"\\
Inverse Problems&\verb"\IP"&Phys. Biol.$^c$&\verb"\PB"\\
J. Breath Res.&\verb"\JBR"&Phys. Educ.$^a$&\verb"\PED"\\
J. Geophys. Eng.$^d$&\verb"\JGE"&Physiol. Meas.$^{c,d,e}$&\verb"\PM"\\
J. Micromech. Microeng.&\verb"\JMM"&Phys. Med. Biol.$^{c,d,e}$&\verb"\PMB"\\
J. Neural Eng.$^c$&\verb"\JNE"&Plasma Phys. Control. Fusion&\verb"\PPCF"\\
J. Opt.&\verb"\JOPT"&Phys. Scr.&\verb"\PS"\\
J. Phys. A: Math. Theor.&\verb"\jpa"&Plasma Sources Sci. Technol.&\verb"\PSST"\\
J. Phys. B: At. Mol. Opt. Phys.&\verb"\jpb"&Rep. Prog. Phys.$^{e}$&\verb"\RPP"\\
J. Phys: Condens. Matter&\verb"\JPCM"&Semicond. Sci. Technol.&\verb"\SST"\\
J. Phys. D: Appl. Phys.&\verb"\JPD"&Smart Mater. Struct.&\verb"\SMS"\\
J. Phys. G: Nucl. Part. Phys.&\verb"\jpg"&Supercond. Sci. Technol.&\verb"\SUST"\\
J. Radiol. Prot.$^a$&\verb"\JRP"&Surf. Topogr.: Metrol. Prop.&\verb"\STMP"\\
Metrologia&\verb"\MET"&Transl. Mater. Res.&\verb"\TMR"\\
$^{a}$UK spelling is required; $^{b}$MSC classification numbers are required; $^{c}$titles of articles are required in journal references; $^{d}$Harvard-style references must be used (see section \ref{except}); $^{e}$final page numbers of articles are required in journal references.


2D Mater.&\verb"\TDM"&J. Radiol. Prot.&\verb"\JRP"\\
AJ&\verb"\AJ"&J. Semicond.&\verb"\JOS"\\
ApJ&\verb"\APJ"&J. Stat. Mech.&\verb"\JSTAT"\\
ApJL&\verb"\APJL"&Laser Phys.&\verb"\LP"\\
ApJS&\verb"\APJS"&Laser Phys. Lett.&\verb"\LPL"\\
Adv. Nat. Sci: Nanosci. Nanotechnol.&\verb"\ANSN"&Metrologia&\verb"\MET"\\
Appl. Phys. Express&\verb"\APEX"&Mater. Res. Express&\verb"\MRE"\\
Biofabrication&\verb"\BF"&Meas. Sci. Technol.&\verb"\MST"\\
Bioinspir. Biomim.&\verb"\BB"&Methods Appl. Fluoresc.&\verb"\MAF"\\
Biomed. Mater.&\verb"\BMM"&Modelling Simul. Mater. Sci. Eng.&\verb"\MSMSE"\\
Chin. J. Chem. Phys.&\verb"\CJCP"&Nucl. Fusion&\verb"\NF"\\
Chinese Phys. B&\verb"\CPB"&New J. Phys.&\verb"\NJP"\\
Chinese Phys. C&\verb"\CPC"&Nonlinearity&\verb"\NL"\\
Chinese Phys. Lett.&\verb"\CPL"&Nanotechnology&\verb"\NT"\\
Class. Quantum Grav.&\verb"\CQG"&Phys. Biol.&\verb"\PB"\\
Commun. Theor. Phys.&\verb"\CTP"&Phys. Educ.&\verb"\PED"\\
Comput. Sci. Disc.&\verb"\CSD"&Phys.-Usp.&\verb"\PHU"\\
Environ. Res. Lett.&\verb"\ERL"&Physiol. Meas.&\verb"\PM"\\
EPL&\verb"\EPL"&Phys. Med. Biol.&\verb"\PMB"\\
Eur. J. Phys.&\verb"\EJP"&Phys. Scr.&\verb"\PS"\\
Fluid Dyn. Res.&\verb"\FDR"&Plasma Phys. Control. Fusion&\verb"\PPCF"\\
Inverse Problems&\verb"\IP"&Plasma Sci. Technol.&\verb"\PST"\\
Izv. Math.&\verb"\IZV"&Plasma Sources Sci. Technol.&\verb"\PSST"\\
Jpn. J. Appl. Phys.&\verb"\JJAP"&Quantum Electron.&\verb"\QEL"\\
J. Breath Res.&\verb"\JBR"&Rep. Prog. Phys.&\verb"\RPP"\\
JCAP&\verb"\JCAP"&Res. Astron. Astrophys.&\verb"\RAA"\\
J. Geophys. Eng.&\verb"\JGE"&Russ. Chem. Rev.&\verb"\RCR"\\
JINST&\verb"\JINST"&Russ. Math. Surv.&\verb"\RMS"\\
J. Micromech. Microeng.&\verb"\JMM"&Sb. Math.&\verb"\MSB"\\
J. Neural Eng.&\verb"\JNE"&Science Foundation in China&\verb"\SFC"\\
J. Opt.&\verb"\JOPT"&Sci. Technol. Adv. Mater.&\verb"\STAM"\\
J. Phys. A: Math. Theor.&\verb"\jpa"&Semicond. Sci. Technol.&\verb"\SST"\\
J. Phys. B: At. Mol. Opt. Phys.&\verb"\jpb"&Smart Mater. Struct.&\verb"\SMS"\\
J. Phys: Condens. Matter&\verb"\JPCM"&Supercond. Sci. Technol.&\verb"\SUST"\\
J. Phys. D: Appl. Phys.&\verb"\JPD"&Surf. Topogr.: Metrol. Prop.&\verb"\STMP"\\
J. Phys. G: Nucl. Part. Phys.&\verb"\jpg"&Transl. Mater. Res.&\verb"\TMR"\\
\mr
{\it IOP Conference Series journals}\\
\mr
J. Phys.: Conf. Ser.&\verb"\JPCS"\\
IOP Conf. Ser.: Earth Environ. Sci.&\verb"\EES"\\
IOP Conf. Ser.: Mater. Sci. Eng.&\verb"\MSE"\\



J. Phys. A: Math. Gen.&\verb"\JPA"&1975--2006\\
J. Phys. B: At. Mol. Phys.&\verb"\JPB"&1968--1987\\
J. Phys. C: Solid State Phys.&\verb"\JPC"&1968--1988\\
J. Phys. E: Sci. Instrum.&\verb"\JPE"&1968--1989\\
J. Phys. F: Met. Phys.&\verb"\JPF"&1971--1988\\
J. Phys. G: Nucl. Phys.&\verb"\JPG"&1975--1988\\
Pure Appl. Opt.&\verb"\PAO"&1992--1998\\
Quantum Opt.&\verb"\QO"&1989--1994\\
Quantum Semiclass. Opt.&\verb"\QSO"&1995--1998\\
J. Opt. A: Pure Appl. Opt.&\verb"\JOA"&1999--2009\\
J. Opt. B: Quantum Semiclass. Opt.&\verb"\JOB"&1999--2005\\



Acta Crystallogr.&\verb"\AC"&J. Quant. Spectrosc. Radiat. Transfer&\verb"\JQSRT"\\
Acta Metall.&\verb"\AM"&Nuovo Cimento&\verb"\NC"\\
Ann. Phys., Lpz&\verb"\AP"&Nucl. Instrum. Methods&\verb"\NIM"\\
Ann. Phys., NY&\verb"\APNY"&Nucl. Phys.&\verb"\NP"\\
Ann. Phys., Paris&\verb"\APP"&Phys. Fluids&\verb"\PF"\\
Can. J. Phys.&\verb"\CJP"&Phys. Lett.&\verb"\PL"\\
Gen. Rel. Grav.&\verb"\GRG"&Phys. Rev.&\verb"\PR"\\
J. Appl. Phys.&\verb"\JAP"&Phys. Rev. Lett.&\verb"\PRL"\\
J. Chem. Phys.&\verb"\JCP"&Proc. R. Soc.&\verb"\PRS"\\
J. High Energy Phys.&\verb"\JHEP"&Phys. Status Solidi&\verb"\PSS"\\
J. Magn. Magn. Mater.&\verb"\JMMM"&Phil. Trans. R. Soc.&\verb"\PTRS"\\
J. Math. Phys.&\verb"\JMP"&Rev. Mod. Phys.&\verb"\RMP"\\
J. Opt. Soc. Am.&\verb"\JOSA"&Rev. Sci. Instrum.&\verb"\RSI"\\
J. Physique&\verb"\JP"&Solid State Commun.&\verb"\SSC"\\
J. Phys. Chem.&\verb"\JPhCh"&Sov. Phys.--JETP&\verb"\SPJ"\\
J. Phys. Soc. Jpn.&\verb"\JPSJ"&Z. Phys.&\verb"\ZP"\\


==> Other_macros.tex <==

\begin{table}[hb]
\caption{Macros available for use in text in {\tt iopart.cls}. Parameters in square brackets are optional.}
\footnotesize\rm
\begin{tabular}{@{}*{7}{l}}
\br
Macro name&Purpose\\
\mr
\verb"\title[#1]{#2}"&Title of article and short title (optional)\\
\verb"\paper[#1]{#2}"&Title of paper and short title (optional)\\
\verb"\letter{#1}"&Title of Letter to the Editor\\
\verb"\ftc{#1}"&Title of Fast Track Communication\\
\verb"\rapid[#1]{#2}"&Title of Rapid Communication and short title (optional)\\
\verb"\comment[#1]{#2}"&Title of Comment and short title (optional)\\
\verb"\topical[#1]{#2}"&Title of Topical Review and short title 
(optional)\\
\verb"\review[#1]{#2}"&Title of review article and short title (optional)\\
\verb"\note[#1]{#2}"&Title of Note and short title (optional)\\
\verb"\prelim[#1]{#2}"&Title of Preliminary Communication \& short title\\
\verb"\author{#1}"&List of all authors\\
\verb"\article[#1]{#2}{#3}"&Type and title of other articles and 
short title (optional)\\
\verb"\address{#1}"&Address of author\\
\verb"\ams{#1}"&Mathematics Classification Scheme\\
\verb"\submitto{#1}"&`Submitted to' message\\
\verb"\maketitle"&Creates title page\\
\verb"\begin{abstract}"&Start of abstract\\
\verb"\end{abstract}"&End of abstract\\
\verb"\nosections"&Inserts space before text when no sections\\
\verb"\section{#1}"&Section heading\\
\verb"\subsection{#1}"&Subsection heading\\
\verb"\subsubsection{#1}"&Subsubsection heading\\
\verb"\appendix"&Start of appendixes\\
\verb"\ack"&Acknowledgments heading\\
\verb"\References"&Heading for reference list\\
\verb"\begin{harvard}"&Start of alphabetic reference list\\
\verb"\end{harvard}"&End of alphabetic reference list\\
\verb"\begin{thebibliography}{#1}"&Start of numeric reference list\\
\verb"\end{thebibliography}"&End of numeric reference list\\
\verb"\etal"&\etal for text and reference lists\\
\verb"\nonum"&Unnumbered entry in numerical reference list\\
\br
\end{tabular}
\end{table}

\clearpage

\begin{table}
\caption{Macros defined within {\tt iopart.cls}
for use with figures and tables.}
\begin{indented}
\item[]\begin{tabular}{@{}l*{15}{l}}
\br
Macro name&Purpose\\
\mr
\verb"\Figures"&Heading for list of figure captions\\
\verb"\Figure{#1}"&Figure caption\\
\verb"\Tables"&Heading for tables and table captions\\
\verb"\Table{#1}"&Table caption\\
\verb"\fulltable{#1}"&Table caption for full width table\\
\verb"\endTable"&End of table created with \verb"\Table"\\
\verb"\endfulltab"&End of table created with \verb"\fulltable"\\
\verb"\endtab"&End of table\\
\verb"\br"&Bold rule for tables\\
\verb"\mr"&Medium rule for tables\\
\verb"\ns"&Small negative space for use in table\\
\verb"\centre{#1}{#2}"&Centre heading over columns\\
\verb"\crule{#1}"&Centre rule over columns\\
\verb"\lineup"&Set macros for alignment in columns\\
\verb"\m"&Space equal to width of minus sign\\
\verb"\-"&Left overhanging minus sign\\
\verb"\0"&Space equal to width of a digit\\
\br
\end{tabular}
\end{indented}
\end{table}

\begin{table}[t]
\caption{\label{blobs}Control sequences to describe lines and symbols in figure 
captions.}
\begin{indented}
\item[]\begin{tabular}{@{}lllll}
\br
Control sequence&Output&&Control sequence&Output\\
\mr
\verb"\dotted"&\dotted        &&\verb"\opencircle"&\opencircle\\
\verb"\dashed"&\dashed        &&\verb"\opentriangle"&\opentriangle\\
\verb"\broken"&\broken&&\verb"\opentriangledown"&\opentriangledown\\
\verb"\longbroken"&\longbroken&&\verb"\fullsquare"&\fullsquare\\
\verb"\chain"&\chain          &&\verb"\opensquare"&\opensquare\\
\verb"\dashddot"&\dashddot    &&\verb"\fullcircle"&\fullcircle\\
\verb"\full"&\full            &&\verb"\opendiamond"&\opendiamond\\
\br
\end{tabular}
\end{indented}
\end{table}


==> instructionstoself.tex <==
PROBLEM WITH AMSMATH.STY?
call main the master file
no subdirectories
EPS files - name them figure1.eps or figure2a.eps etc 
no punctuation in file names
Captions end with .

Use -ize spellings
Don't use Eq. or equation before an equation number or ref. before a reference number.

Leave $\lambda/2\pi$ but \frac12 for simple fractions

No subcaptions, just empty (a) (b) (c)

REFS
 For the numerical (Vancouver) reference style we recommend that authors use  \verb"unsrt.bst"; this does not quite follow the style of published articles in our journals but this is not a problem.  Alternatively \verb"iopart-num.bst" created by Mark A Caprio produces a reference style that closely matches that in published articles.  The file is available from
\verb"http://ctan.org/tex-archive/biblio/bibtex/contrib/iopart-num/" .
\item For alphabetical (Harvard) style references we recommend that authors use the \verb"harvard.sty"
in conjunction with the \verb"jphysicsB.bst" BibTeX style file.  These, and accompanying documentation, can be downloaded from \penalty-10000 \verb"http://www.ctan.org/tex-archive/macros/latex/contrib/harvard/".
Note that the \verb"jphysicsB.bst" bibliography style does not include article titles in references to journal articles. To include the titles of journal articles you can use the style \verb"dcu.bst" which is included in the \verb"harvard.sty" package.  The output differs a little from the final journal reference style, but all of the necessary information is present and the reference list will be formatted into journal house style as part of the production process if your article is accepted for publication.
